ChatGPT for Robotics: Design Principles and Model Abilities

This paper presents an experimental study regarding the use of OpenAI's ChatGPT for robotics applications. We outline a strategy that combines design principles for prompt engineering and the creation of a high-level function library which allows ChatGPT to adapt to different robotics tasks, simulators, and form factors. We focus our evaluations on the effectiveness of different prompt engineering techniques and dialog strategies towards the execution of various types of robotics tasks. We explore ChatGPT's ability to use free-form dialog, parse XML tags, and to synthesize code, in addition to the use of task-specific prompting functions and closed-loop reasoning through dialogues. Our study encompasses a range of tasks within the robotics domain, from basic logical, geometrical, and mathematical reasoning all the way to complex domains such as aerial navigation, manipulation, and embodied agents. We show that ChatGPT can be effective at solving several of such tasks, while allowing users to interact with it primarily via natural language instructions. In addition to these studies, we introduce an open-sourced research tool called PromptCraft, which contains a platform where researchers can collaboratively upload and vote on examples of good prompting schemes for robotics applications, as well as a sample robotics simulator with ChatGPT integration, making it easier for users to get started with using ChatGPT for robotics.

==> inputs/prompts/diff_apis.tex <==
% !TEX root = ../../root.tex
{\scriptsize	
\begin{mdframed}
\user{
Consider you are a home assistant robot. You goal is to prepare an omelette for an elderly person. You are equipped with functions:\\
\function{locate\_object(obj\_name)}: returns a X,Y,Z tuple representing the location of the desired object defined by string "obj\_name";\\
\function{move\_to\_location(X,Y,Z)}: moves the robot's hands to a specific X,Y,Z location in space. Returns nothing;\\
\function{cook\_item(obj\_name)}: cooks a particular item defined by "obj\_name". Returns nothing;\\
\function{grab\_object(obj\_name)}: picks a particular object defined by "obj\_name". Returns nothing;\\
Output python code with the sequence of steps that achieves your objective.\\
}
\llm{
Sure, here is an example Python code that utilizes the provided functions to prepare an omelette for an elderly person:\\
\codebox{
\# Define the names of the objects needed for the omelette
EGGS = "eggs"\\
BOWL = "bowl"\\
PAN = "pan"\\
OIL = "oil"\\
eggs\_location = locate\_object(EGGS)\\
bowl\_location = locate\_object(BOWL)\\
pan\_location = locate\_object(PAN)\\
oil\_location = locate\_object(OIL)\\
\# Move the robot's hands to the bowl location and grab the eggs\\
move\_to\_location(bowl\_location)\\
grab\_object(EGGS)\\
\# Move the robot's hands to the pan location and add oil\\
move\_to\_location(pan\_location)\\
grab\_object(OIL)\\
\# Move the robot's hands to the bowl location and crack the eggs into the bowl\\
move\_to\_location(bowl\_location)\\
cook\_item(EGGS)\\
\# Move the robot's hands to the pan location and pour the eggs into the pan\\
move\_to\_location(pan\_location)\\
cook\_item(BOWL)\\
\# Wait for the omelette to cook\\
\# (I'm assuming the cook\_item function takes care of this step)\\
\# Serve the omelette\\
\# (I'm assuming the cook\_item function takes care of this step)
}
}
\end{mdframed}
}


==> inputs/prompts/logical_reasoning.tex <==
% !TEX root = ../../root.tex

{
\scriptsize	
\begin{mdframed}
\user{Imagine we are working with a robot arm. I have two platforms separated by a distance, and a tub of water in between. I need to be able to roll a ball from one platform to the other. We also have several plastic blocks lying around. How can we achieve this with the arm?}\\
\llm{One way to achieve this with a robot arm is to use the plastic blocks to build a bridge across the tub of water. Once the bridge is in place, the robot arm can roll the ball from one platform to the other by carefully placing it on the bridge.
Here's the step-by-step process:
Pick up the first plastic block with the robot arm.
Place the block on the first platform, near the edge of the tub of water.
Repeat the process of picking up a block and placing it next to the previous block, until a bridge is formed that spans the tub of water.
Use the robot arm to roll the ball onto the bridge.
Use the robot arm to guide the ball across the bridge to the second platform.
It's important to make sure that the bridge is stable and can support the weight of the ball. You may need to adjust the number and placement of blocks to ensure a stable bridge.
}
\user{Imagine there is another household robot that is trying to go through a hallway. The entrance to the hallway is blocked by a big box. The robot does not have arms to pick up and move the box. It can only move forward, or turn left/right. There are no alternative routes. What can it do to move the box so it can enter the hallway?}
\llm{In this scenario, the household robot may be able to move the box by pushing it. However, since the robot does not have arms, it will need to use its body to push the box.
Here's the step-by-step process the robot can follow to move the box:
Approach the box from the side.
Position the front of the robot's body against the side of the box.
Slowly apply force to the box, pushing it in the desired direction.
Continue pushing the box until it moves out of the way of the hallway entrance.
Once the box has been moved, the robot can enter the hallway.
It's important to be careful when pushing the box, as the robot needs to maintain its balance and stability while pushing. The speed and force of the push will also need to be carefully controlled to ensure that the box moves in a controlled manner, without tipping over or causing damage.}

\end{mdframed}
}






==> inputs/prompts/manip_curriculum.tex <==
% !TEX root = ../../root.tex
{\scriptsize	
\begin{mdframed}
$[$Initial model prompt found in Appendix~\ref{subsec:appendix_manip_curriculum}$]$\\
$[$The beginning of the conversation is omitted for brevity. The following excerpt requires ChatGPT to build a new function using previously defined APIs, and later use this function for more complex tasks.$]$\\
\user{I want you to learn how to place an object in a position. Considering you are holding a generic object, you first need to first move to a safe position above the target location, bring the object down and then release it.}
\breaktext{}
\llm{Understood. Here's a Python function that takes the position where the object should be placed, moves the robot arm above the position, brings the object down, and releases it. Note that the function assumes that the robot arm is holding an object.}
\begin{lstlisting}[language=Python]
def place_object(position):
    # move the robot arm to a safe position above the target location
    safe_pos = [position[0], position[1], position[2]+100, position[3], position[4], position[5]]
    move_to(safe_pos)
    # move the robot arm to the target location
    move_to(position)
    # release the object
    release()
    # move the robot arm back to the safe position above the target location
    move_to(safe_pos)
\end{lstlisting}
\user{Awesome! I want now to use the blocks to build the logo from Microsoft on top of the white pad. It consists of four colors forming a square, blue on the bottom left, yellow on the bottom right, red on the top left and green on the top right.}
\breaktext{}
\llm{Sure! Here's the Python code to build the Microsoft logo on top of the white pad using the blocks:\\
\breaktext{}
$[$Code not show for brevity. Please consult the link for the full conversation$]$\\
\breaktext{}
This code gets the positions of the white pad and all four blocks using the get\_position function, picks up each block in turn using the pick\_up\_object function we defined earlier, calculates the position to place the block on the white pad, and places the block on the white pad using the place\_object function we defined earlier. We use the block colors to ensure that the logo is built correctly. We place the blue block in the bottom left position, the yellow block in the bottom right position, the red block in the top left position, and the green block in the top right position, as specified in the prompt.\\
\begingroup\normalfont
  \includegraphics[height=50px]{figs/manip_seq}%
  \endgroup
  \ [\textit{snapshots from \href{https://github.com/microsoft/PromptCraft-Robotics}{manipulator video}}]
  }
\end{mdframed}
}


==> inputs/prompts/multiple_robots.tex <==
% !TEX root = ../../root.tex

{
\scriptsize	
\begin{mdframed}
$[$initial model prompt found in Appendix~\ref{subsec:appendix_multipe_robots}$]$\\
\user{Let us assume the X axis is facing east, and Y axis is facing north. All three agents start at (0,0,0), facing north. Give me code that can move all three agents from the XYZ coordinates (0, 0, 0) to (5, 5, 0). Add comments to the code explaining what you are doing, and keep the code compact and correctly formatted.}
\begin{lstlisting}[language=Python]
# Embodied agent
def move_embodied_agent_to_target(x, y):
  # rotate to face east
  turn_right()  
  # move forward until we reach the target x position
  while x > 0:
    move_forward()
    x -= 1  
  # rotate to face north
  turn_left()  
  # move forward until we reach the target y position
  while y > 0:
    move_forward()
    y -= 1
    
move_embodied_agent_to_target(5, 5)

# Small car
def move_car_to_target(x, y):
  # get the initial position
  current_pos = get_position()
  target_pos = (x, y, 0)  
  # calculate the angle to target position
  angle = math.atan2(target_pos[1]-current_pos[1], target_pos[0]-current_pos[0])  
  # set initial steering angle
  set_steering_angle(angle)
  set_velocity(1)  
  # continuously update the steering angle as the car moves
  while current_pos[0] != target_pos[0] or current_pos[1] != target_pos[1]:
    current_pos = get_position()
    angle = math.atan2(target_pos[1]-current_pos[1], target_pos[0]-current_pos[0])
    set_steering_angle(angle)
    # stop the car
  set_velocity(0)

move_car_to_target(5, 5)

# Drone
def move_drone_to_target(x, y, z):
  # take off
  set_height(1)  
  # fly to the target x and y position
  angle = math.atan2(y, x)
  set_yaw(angle)
  set_pitch(45)  
  # continuously update the drone position
  current_pos = get_position()
  while current_pos[0] != x or current_pos[1] != y:
    current_pos = get_position()
  # fly to the target z position
  set_pitch(0)
  set_height(z)  
  # land
  set_height(0)

move_drone_to_target(5, 5, 0)
\end{lstlisting}
\end{mdframed}
}




==> inputs/prompts/new_apis.tex <==
% !TEX root = ../../root.tex
{\scriptsize	
\begin{mdframed}
\user{
Consider you are a home assistant robot. You goal is to prepare an omelette for an elderly person. You are equipped with functions:\\
\function{locate\_object(obj\_name)}: returns a X,Y,Z tuple representing the location of the desired object defined by string "obj\_name";\\
\function{move\_to\_location(X,Y,Z)}: moves the robot's hands to a specific X,Y,Z location in space. Returns nothing;\\
\function{cook\_item(obj\_name)}: cooks a particular item defined by "obj\_name". Returns nothing;\\
\function{grab\_object(obj\_name)}: picks a particular object defined by "obj\_name". Returns nothing;\\
Output python code with the sequence of steps that achieves your objective. You can define other new functions in the beginning of the code if they are useful for the task.
}
\breaktext{}
\llm{
\codebox{
def crack\_eggs(num\_eggs):\\
\hspace*{4mm} for i in range(num\_eggs):\\
\hspace*{4mm}\hspace*{4mm}grab\_object("egg")\\
\hspace*{4mm}\hspace*{4mm}move\_to\_location(10, 10, 0)\\
\hspace*{4mm}\hspace*{4mm}cook\_item("egg")\\
\hspace*{4mm}\hspace*{4mm}move\_to\_location(0, 0, 0)\\
def chop\_veggies(veggie\_name):\\
\hspace*{4mm}location = locate\_object(veggie\_name)\\
\hspace*{4mm}move\_to\_location(location[0], location[1], location[2])\\
\hspace*{4mm}for i in range(3):\\
\hspace*{4mm}\hspace*{4mm}grab\_object(veggie\_name)\\
\hspace*{4mm}\hspace*{4mm}move\_to\_location(i*5, 5, 0)\\
\hspace*{4mm}\hspace*{4mm}move\_to\_location(0, 0, 0)\\
}
\breaktext{}
\lbrack \textit{remainder of the answer omitted for brevity} \rbrack
}
\end{mdframed}
}


==> inputs/prompts/prompt_tello.tex <==
{\footnotesize	
\begin{mdframed}
  \user{
Imagine you are helping me interact with the AirSim simulator for drones. At any given point of time, you have the following abilities, each identified by a unique tag. You are also required to output code for some of the requests.
\breaktext{}
Question: You can ask me a clarification question, as long as you specifically identify it saying "Question".\\
Code: Output a code command that achieves the desired goal.\\  
Reason: After you output code, you should provide an explanation why you did what you did.
\breaktext{}
The simulator contains a drone, along with several objects. Apart from the drone, none of the objects are movable. Within the code, we have the following commands available to us. You are not to use any other hypothetical functions.
\breaktext{}
\function{get\_position(object\_name)}: Takes a string as input indicating the name of an object of interest, and returns a vector of 4 floats indicating its X,Y,Z,Angle coordinates.\\
\function{self.tello.fly\_to(position)}: Takes a vector of 4 floats as input indicating X,Y,Z,Angle coordinates and commands the drone to fly there and look at that angle\\
\function{self.tello.fly\_path(positions)}: Takes a list of X,Y,Z,Angle positions indicating waypoints along a path and flies the drone along that path\\
\function{self.tello.look\_at(angle)}: Takes an angle as input indicating the yaw angle the drone should look at, and rotates the drone towards that angle
\breaktext{}
Here is an example scenario that illustrates how you can ask clarification questions. Let us assume a scene contains two spheres?
\breaktext{}
Me: Fly to the sphere.\\
You: Question there are two spheres. Which one do you want me to fly to?\\
Me: Sphere 1, please.
\breaktext{}
You also have access to a Python dictionary whose keys are object names, and values are the X,Y,Z,Angle coordinates for each object:
\breaktext{}
self.dict\_of\_objects = \{'origin': [0.0, 0.0, 0.0, 0],
                                'mirror': [1.25, -0.15, 1.2, 0],
                                'chair 1': [0.9, 1.15, 1.1, np.pi/2],
                                'orchid': [0.9, 1.65, 1.1, np.pi/2],
                                'lamp': [1.6, 0.9, 1.2, np.pi/2],
                                'baby ducks': [0.1, 0.8, 0.8, np.pi/2],
                                'sanitizer wipes': [-0.3, 1.75, 0.9, 0],
                                'coconut water': [-0.6, 0.0, 0.8, -np.pi],
                                'chair 2': [-0.8, -0.8, 1.1, np.pi],
                                'computer': [-1.5, -0.8, 1.1, np.pi],
                                'shelf': [0.95, -0.9, 1.2, np.pi/2],
                                'diet coke can': [1.0, -0.9, 1.55, np.pi/2],
                                'regular coke can': [1.3, -0.9, 1.55, np.pi/2]\}
\breaktext{}                               
Are you ready?
}
  \breaktext{} 
  \llm{Yes, I am ready! Please provide the request you would like me to fulfill.}
  \breaktext{}
  \user{I am thirsty. Find me a drink}
  \breaktext{}
  \llm{Question: What kind of drink are you looking for? Question: What kind of drink are you looking for?Question: What kind of drink are you looking for?Question: What kind of drink are you looking for?Question: What kind of drink are you looking for?Question: What kind of drink are you looking for?}
  \breaktext{}
  \user{I just came back from the gym and am looking for a healthy option.}
  \breaktext{}
  \llm{Question: Can you provide more specific information on the healthy drink you are looking for?}
  \breaktext{}
  \user{Any healthy option from the environment}
  \breaktext{}
  % \llm{
  % 	\fbox{\footnotesize	
% 	\begin{minipage}{\textwidth}
% 	  blabla
% 	\end{minipage}
  % }
  \llm{
  	Code:
  	\breaktext{}
  	\codebox{
  		drink = 'coconut water'\\
		position = self.dict\_of\_objects[drink]\\
        self.tello.fly\_to(position)
        }
    \breaktext{}
    Reason:\\
	We use the dictionary self.dict\_of\_objects to retrieve the coordinates of the object "coconut water". We then use the fly\_to method to fly the drone to that position.
  }
  \breaktext{}
  \user{I am still thirsty and craving sugar. Can you find another one?}
  \breaktext{}
  \llm{
  Code:
  \breaktext{}
  	\codebox{
  		drink = 'diet coke can'\\
		position = self.dict\_of\_objects[drink]\\
		self.tello.fly\_to(position)
        }
    \breaktext{}
    Reason:\\
	We use the dictionary self.dict\_of\_objects to retrieve the coordinates of the object "diet coke can". We then use the fly\_to method to fly the drone to that position.
  }
  \breaktext{}
  \user{Does diet coke have sugar?}
  \breaktext{}
  \llm{Diet coke is a low calorie or sugar-free alternative to regular Coca Cola. It typically uses artificial sweeteners such as aspartame or acesulfame potassium instead of sugar to provide the sweet taste, but it does not contain any actual sugar.}
  \breaktext{}
  \user{Then why did you go there? }
  \breaktext{}
  \llm{My apologies, I made a mistake. Diet Coke is not a sugary drink. You specified that you were looking for a drink with sugar, but Diet Coke is a sugar-free alternative. Let me know what would you like me to do next.}
  \breaktext{}
  \user{Find a drink with sugar}
  \breaktext{}
  \llm{
  Code:
  \breaktext{}
  	\codebox{
  		drink = 'regular coke can'\\
		position = self.dict\_of\_objects[drink]\\
		self.tello.fly\_to(position)
        }
  }
  \breaktext{}
  \user{Take a selfie using a reflective surface.}
  \breaktext{}
\end{mdframed}
}


==> inputs/prompts/robotics_scripts.tex <==
% !TEX root = ../../root.tex

{
\scriptsize	
\begin{mdframed}
\user{Imagine we are working with a robot car that is equipped with a camera operating in a two dimensional space. Let us also assume there is an object detection model running on the robot that is able to detect an object of interest in the camera's image, and pass the pixel coordinates of the center of the object at every timestep. This object is in motion but only along the horizontal axis. 
The robot always moves forward at a constant velocity, but the yaw angle can be controlled by the function set_angle(). is_reached() is a function that checks whether the robot has reached the object. Can you write code for a controller that reactively controls the robot such that the object is always directly in front of the robot?
}\\
\begin{lstlisting}[language=Python]
def controller(pixel_x):
    # Set a target x-coordinate for the object
    target_x = image_width / 2
    
    # Calculate error between current and target x-coordinate
    error = target_x - pixel_x
    
    # Set a proportionate gain for the control loop
    kp = 0.01
    
    # Calculate the angle to set based on the error and the gain
    angle = kp * error
    
    # Call the set_angle function to adjust the yaw angle
    set_angle(angle)
    
    # Check if the object has been reached
    if is_reached():
        return True
    else:
        return False
\end{lstlisting}    
\llm{The code above implements a simple proportional control loop that continuously adjusts the yaw angle of the robot such that the object remains directly in front of the robot. The error is calculated as the difference between the target x-coordinate (the center of the image) and the current x-coordinate of the object. The gain kp determines how much the angle should be adjusted based on the error, with a larger gain leading to a more aggressive correction. The function set_angle is called with the calculated angle to adjust the yaw angle of the robot. The function is_reached is checked to see if the object has been reached, and the controller returns True if the object has been reached, or False if the object has not yet been reached.}
\end{mdframed}
}



